DVP: Data Visualization Platform

We identify two major steps in data analysis, data exploration for understanding and observing patterns/relationships in data; and construction, design and assessment of various models to formalize these relationships. For each step, there exists a large set of tools and software. For the first step, many visualization tools exist, such as, GGobi, Parallax, and Crystal Vision, and most recently tableau and plottly. For the second step, many Scientific Computing Environments (SCEs) exist, such as, Matlab, Mathematica, R and Python. However, there does not exist a tool which allows for seamless two-way interaction between visualization tools and SCEs. We have designed and implemented a data visualization platform (DVP) with an architecture and design that attempts to bridge this gap. DVP connects seamlessly to SCEs to bring the computational capabilities to the visualization methods in a single coherent platform. DVP is designed with two interfaces, the desktop stand alone version and the online interface. To illustrate the power of DVP design, a free demo for the online interface of DVP is available \citep{DVP} and very low-level design details are explained in this article. Since DVP was launched, circa 2012, the present manuscript was not published since today for commercialization and patent considerations.

==> secabstract.tex <==
We identify two major steps in data analysis, data exploration for understanding and observing
patterns/relationships in data; and construction, design and assessment of various models to
formalize these relationships. For each step, there exists a large set of tools and software. For
the first step, many visualization tools exist, such as, GGobi, Parallax, and Crystal Vision, and
most recently tableau and plottly. For the second step, many Scientific Computing Environments
(SCEs) exist, such as, Matlab, Mathematica, R and Python. However, there does not exist a tool which
allows for seamless two-way interaction between visualization tools and SCEs. We have designed and
implemented a data visualization platform (DVP) with an architecture and design that attempts to
bridge this gap. DVP connects seamlessly to SCEs to bring the computational capabilities to the
visualization methods in a single coherent platform. DVP is designed with two interfaces, the
desktop stand alone version and the online interface. DVP with its structure and planned features is
a unique software that serves a great deal of parties, including university research, governmental
decision support and country's economy modeling, traffic analysis and control, financial sector and
companies, and any other party interested in data analysis and interpretation. A free demo for the
online interface of DVP is available \citep{DVP}. Since DVP was launched, circa 2012, the present
manuscript was not published since today for commercialization and patent considerations.
